Sparse Deep Learning for Time Series Data: Theory and Applications

Sparse deep learning has become a popular technique for improving the performance of deep neural networks in areas such as uncertainty quantification, variable selection, and large-scale network compression. However, most existing research has focused on problems where the observations are independent and identically distributed (i.i.d.), and there has been little work on the problems where the observations are dependent, such as time series data and sequential data in natural language processing. This paper aims to address this gap by studying the theory for sparse deep learning with dependent data. We show that sparse recurrent neural networks (RNNs) can be consistently estimated, and their predictions are asymptotically normally distributed under appropriate assumptions, enabling the prediction uncertainty to be correctly quantified. Our numerical results show that sparse deep learning outperforms state-of-the-art methods, such as conformal predictions, in prediction uncertainty quantification for time series data. Furthermore, our results indicate that the proposed method can consistently identify the autoregressive order for time series data and outperform existing methods in large-scale model compression. Our proposed method has important practical implications in fields such as finance, healthcare, and energy, where both accurate point estimates and prediction uncertainty quantification are of concern.

==> figures_tables/datasets.tex <==
\begin{table}[t]
\caption{A brief description of the three datasets used in Section \ref{main: exp_set_of_ts}. The Train size and Test size columns indicate the number of training and testing sequences, respectively. The Length column represents the length of the input sequence.}
\label{table: datasets}
\begin{center}
\begin{tabular}{ c c c c c} 
\toprule
\textbf{Dataset} & \textbf{Train size} & \textbf{Test size} & \textbf{Length} & \textbf{Prediction horizon}\\
\midrule
MIMIC-III \cite{johnson2016mimic} & $2692$ & $300$ & $[3, 47]$ & $2$\\
EEG \cite{blake1998uci} & $19200$ & $19200$ & $40$ & $10$\\
COVID-19 \cite{uk2020coronavirus} & $300$ & $80$ & $100$ & $50$\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> figures_tables/simulation.tex <==
\begin{table}[t]
\caption{Simulation results: numbers inside the parentheses are the corresponding standard deviations, "-" indicates not applicable, and $\downarrow$ means lower is better. All results are obtained from five independent runs. The number after the model name represents the input window size, i.e., PA-RNN $15$ uses a window size of $15$.}
\label{table: sim_results}
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ c | c c c c c c} 
\toprule
Model & FSR $\downarrow$ & NSR $\downarrow$ & AR order & \# non-zero hidden connections & MSPE $\downarrow$ & MSFE $\downarrow$ \\
\midrule
PA-RNN $1$ & - & - & - & $357(48)$ & $1.056(0.022)$ & $1.057(0.014)$\\

PA-RNN $15$ & $0.23$ & $0$ & $7.4(0.49)$ & $0(0)$ & $1.017(0.017)$ & $1.020(0.023)$ \\

RNN $1$ & - & - & - & - & $1.090(0.014)$ & $1.090(0.021)$\\

RNN $15$ & - & - & - & - &  $1.040(0.011)$ & $1.046(0.015)$\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> figures_tables/uc_fesp.tex <==
\begin{table}[t]
\caption{Uncertainty quantification performance of different methods on the French electricity spot prices dataset.This table corresponds to the Figure \ref{fig: fesp_results}. Values in parentheses indicate the standard deviations of the respective means.}
\label{table: fesp_results}
\begin{center}
\begin{tabular}{c | c | c } 
\toprule
Methods & Coverage & PI Lengths\\
\midrule
PA offline  & $90.06$ & $20.19(3.23)$ \\
AgACI online  & $91.05$ & $23.27(14.49)$ \\
ACI $\gamma=0.01$ online & $90.21$ & $22.13(8.50)$\\
ACI $\gamma=0.0$ online & $92.89$ & $24.39(9.17)$\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> figures_tables/uc_set_ts.tex <==
\begin{table}[t]
\caption{Uncertainty quantification results by different methods for the MIMIC-III, EEG and COVID-19 data, where ``Coverage'' represents the joint coverage rate averaged over different   random seeds, the prediction interval length is averaged across prediction horizons and random seeds, and the numbers in the parentheses indicate the standard deviations of the respective means.}
\label{table: set_of_ts_results}
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}c | c c | c c | c c @{}}
\toprule
\multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{MIMIC-III}} & \multicolumn{2}{c}{\textbf{EEG}}  & \multicolumn{2}{c}{\textbf{COVID-19}}\\
\midrule
\multicolumn{1}{l}{\textbf{Model}} & Coverage & PI lengths & Coverage & PI lengths & Coverage & PI lengths\\
\midrule
PA-RNN  & $90.8\%(1.5\%)$ & $2.35(0.26)$ & $94.69\%(1.0\%)$ & $51.02(10.50)$ & $90.5\%(3.3\%)$ & $444.93(203.28)$\\
CF-RNN  & $92.0\%(0.7\%)$ & $3.01(0.17)$ & $96.5\%(1.0\%)$ & $61.86(18.02)$&  $89.7\%(5.3\%)$ & $733.95(582.52)$\\
MQ-RNN  & $85.3\%(0.5\%)$ & $2.64(0.11)$ & $48.0\%(4.0\%)$ & $21.39(2.36)$ &$15.0\%(5.9\%)$ & $136.56(63.32)$\\
DP-RNN  & $1.2\%(0.7\%)$  & $0.12(0.01)$ & $3.3\%(0.7\%)$ & $7.39(0.74)$ & $0.0\%(0.0\%)$ & $61.18(32.37)$\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}
